Distributed optimization decomposition for joint economic dispatch and frequency regulation

Economic dispatch and frequency regulation are typically viewed as fundamentally different problems in power systems and, hence, are typically studied separately. In this paper, we frame and study a joint problem that co- optimizes both slow timescale economic dispatch resources and fast timescale frequency regulation resources. We show how the joint problem can be decomposed without loss of optimality into slow and fast timescale sub-problems that have appealing interpretations as the economic dispatch and frequency regulation problems respectively. We solve the fast timescale sub-problem using a distributed frequency control algorithm that preserves the stability of the network during transients. We solve the slow timescale sub-problem using an efficient market mechanism that coordinates with the fast timescale sub-problem. We investigate the performance of the decomposition on the IEEE 24-bus reliability test system.

==> relatedwork.tex <==
%!TEX root = root.tex
\subsection{Related literature}
\adam{Add this if we have more to say about related papers than we feel like including into the Regulation and Market sections.} 

\enrique{I don't think this is needed, given the references in other places.}


